Some Insights into the Geometry and Training of Neural Networks

Neural networks have been successfully used for classification tasks in a rapidly growing number of practical applications. Despite their popularity and widespread use, there are still many aspects of training and classification that are not well understood. In this paper we aim to provide some new insights into training and classification by analyzing neural networks from a feature-space perspective. We review and explain the formation of decision regions and study some of their combinatorial aspects. We place a particular emphasis on the connections between the neural network weight and bias terms and properties of decision boundaries and other regions that exhibit varying levels of classification confidence. We show how the error backpropagates in these regions and emphasize the important role they have in the formation of gradients. These findings expose the connections between scaling of the weight parameters and the density of the training samples. This sheds more light on the vanishing gradient problem, explains the need for regularization, and suggests an approach for subsampling training data to improve performance.

==> macros.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%        macros.tex                                  %
%                                                    %
% Current version: Michael P. Friedlander            %
%                  Dept of Computer Science          %
%                  University of British Columbia    %
%                                                    %
% 1998: Derived from Michael Saunders's macros file. %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% $Revision: 1.2 $ $Date: 2004-04-20 10:18:51-05 $
% 13 Mar 1999: Added Abract environment
% 11 May 2000: Added several theorem environments
% 08 Jun 2001: Deleted absract environment
% 09 Nov 2001: Using RequirePackage to load req'd packages
% 21 Mar 2004: Deleted lots of never-used macros.  Cleanup.
% 06 Jul 2005: Using mathbb instead of mathds.  Looks better.

%%%%%%%%%%%
%  Packages
%%%%%%%%%%%
\RequirePackage{amsmath}
\RequirePackage{amssymb}
%\RequirePackage{dsfont}

%%%%%%%%%%%%%%%%%%%
% -- AMSMATH tweak:
% Subassumptions environment similar to subequations.
%%%%%%%%%%%%%%%%%%%
\makeatletter
\newcounter{parenttheorem}%
\newenvironment{subassumptions}{%
  \refstepcounter{theorem}%
  \protected@edef\theparenttheorem{\thetheorem}%
  \setcounter{parenttheorem}{\value{theorem}}%
  \setcounter{theorem}{0}%
  \def\thetheorem{\theparenttheorem\normalfont\alph{theorem}}%
  \ignorespaces
}{%
  \setcounter{theorem}{\value{parenttheorem}}%
  \ignorespacesafterend
}
\makeatother

%%%%%%%%%%%%%%%%%%%
% BibTeX macro.  Taken from /usr/share/texmf/doc/bibtex/base/btxdoc.tex.
%%%%%%%%%%%%%%%%%%%
\def\BibTeX{{\rm B\kern-.05em{\sc i\kern-.025em b}\kern-.08em
    T\kern-.1667em\lower.7ex\hbox{E}\kern-.125emX}}
\def\tild{\raisebox{-0.5ex}{\~{}}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Minimize, maximize, subject to
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\minim{\mathop{\hbox{minimize}}}
\def\maxim{\mathop{\hbox{maximize}}}
\def\minimize#1{\displaystyle\minim_{#1}}
\def\maximize#1{\displaystyle\maxim_{#1}}
\def\st{\mathop{\hbox{subject to}}}
\def\argmin{\mathop{\rm arg\,min}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Max/Min Problems
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\makeatletter
\def\uncprob#1#2#3{\fbox
  {\begin{tabular*}{0.84\textwidth}
      {@{}l@{\extracolsep{\fill}}l@{\extracolsep{9pt}}l@{\extracolsep{\fill}}l@{}}
      #1 & $\minimize{#2}$ & $#3$ & $ $
    \end{tabular*}}}
\def\problem#1#2#3#4{\fbox
  {\begin{tabular*}{0.84\textwidth}
      {@{}l@{\extracolsep{\fill}}l@{\extracolsep{6pt}}l@{\extracolsep{\fill}}l@{}}
      #1 & $\minimize{#2}$ & $#3$ & $ $ \\[5pt]
         & $\st          $ & $#4$ & $ $
    \end{tabular*}}}
\def\problemnb#1#2#3#4{
  {\begin{tabular*}{0.84\textwidth}
      {@{}l@{\extracolsep{\fill}}l@{\extracolsep{6pt}}l@{\extracolsep{\fill}}l@{}}
      #1 & $\minimize{#2}$ & $#3$ & $ $ \\[5pt]
         & $\st          $ & $#4$ & $ $
    \end{tabular*}}}
\def\probwide#1#2#3#4{\fbox
  {\begin{tabular*}{.98\textwidth}
      {@{}l@{\extracolsep{\fill}}l@{\extracolsep{6pt}}l@{\extracolsep{\fill}}l@{}}
      #1 & $\minimize{#2}$ & $#3$ & $ $ \\[5pt]
         & $\st          $ & $#4$ & $ $
    \end{tabular*}}}
\def\probnarrow#1#2#3#4{\fbox
  {\begin{tabular*}{0.7\paperwidth}
      {@{}l@{\extracolsep{\fill}}c@{\extracolsep{6pt}}l@{\extracolsep{\fill}}l@{}}
      #1 & $\minimize{#2}$ & $#3$ & $ $ \\[5pt]
         & $\st          $ & $#4$ & $ $
    \end{tabular*}}}
\makeatother

\def\dps\displaystyle
\def\clink#1{\mkern2mu\overline{\mkern-2mu c\mkern2mu}\mkern-2mu\k(#1)}
\def\ul#1{\underline{#1}}
\def\Real{\mathbb{R}}
\def\Symm{\mathbb{S}}
\def\Complex{\mathds{C}}
\def\m{\phantom-}
%\def\eval#1#2{\left.#2\right|_{\alpha=#1}}
% Matrices and vectors
%\def\tmat#1#2{(\, #1 \ \ #2 \,)}
%\def\tmatt#1#2#3{(\, #1 \ \  #2 \ \  #3\,)}
%\def\tmattt#1#2#3#4{(\, #1 \ \  #2 \ \  #3 \ \  #4\,)}
%\def\mat#1#2{(\; #1 \quad #2 \;)}
%\def\matt#1#2#3{(\; #1 \quad #2 \quad #3\;)}
%\def\mattt#1#2#3#4{(\; #1 \quad #2 \quad #3 \quad #4\;)}
\def\pmat#1{\begin{pmatrix}#1\end{pmatrix}}
\def\bmat#1{\begin{bmatrix}#1\end{bmatrix}}
\def\comp#1#2{[#2]_{#1}}
\def\compi#1{[#1]_i}
\def\compj#1{[#1]_j}
%\def\defd{\raisebox{-.2ex}{$\stackrel{\mathrm{def}}{=}$}}
\def\defd{\mathrel{\mathop:}=} % As per Higham's ``Accuracy & Stability...''
\def\abs#1{|#1|}
\def\norm#1{\|#1\|}
\def\onenorm#1{\|#1\|_1}
\def\twonorm#1{\|#1\|_2}
\def\infnorm#1{\norm{#1}_\infty}
\def\blackslug{\hbox{\hskip 1pt \vrule width 4pt height 6pt depth 1.5pt
  \hskip 1pt}}
\def\cross{{\scriptscriptstyle\times}}
\def\cond{\hbox{\rm cond}}
\def\det{\mathop{\hbox{\rm det}}}
\def\diag{\mathop{\hbox{\rm diag}}}
\def\dim{\mathop{\hbox{\rm dim}}}  
\def\boundary{\mathop{\hbox{\rm bnd}}}
\def\interior{\mathop{\hbox{\rm int}}}
\def\Null{\mathop{\hbox{\rm null}}}
\def\rank{\mathop{\hbox{\rm rank}}}
\def\op{\mathop{\hbox{\rm op}}}
\def\range{\mathop{\hbox{\rm range}}}
\def\sign{\mathop{\hbox{\rm sign}}}
\def\sgn{\mathop{\hbox{\rm sgn}}}
\def\Span{\mbox{\rm span}}
\def\trace{\mathop{\hbox{\rm trace}}}
\def\drop{^{\null}}
\def\float{fl}
\def\grad#1{\nabla_{#1}}
\def\Hess#1{\nabla^2_{#1}}
\def\one{\mathbf{1}}
\def\half{{\textstyle{\frac{1}{2}}}}
\def\third{{\textstyle{\frac{1}{3}}}}
\def\fourth{{\textstyle{\frac{1}{4}}}}
\def\sfrac#1#2{{\textstyle{\frac{#1}{#2}}}}
\def\inv{^{-1}}
\def\invsq{^{-2}}
\def\limk{\lim_{k\to\infty}}
\def\mystrut{\vrule height10.5pt depth5.5pt width0pt}
\def\spose#1{\hbox to 0pt{#1\hss}}
\def\sub#1{^{\null}_{#1}}
\def\text #1{\hbox{\quad#1\quad}}
\def\textt#1{\hbox{\qquad#1\qquad}}
\def\invT{^{-T}\!}
\def\T{^T\!}
\def\pT{^{+T}}
\def\xint{{x_{\rm int}}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%  Fixed-size glue, only for math mode
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\pthinsp{\mskip  2   mu}    %           thin space
\def\pmedsp {\mskip  2.75mu}    %         medium space
\def\pthiksp{\mskip  3.5 mu}    %          thick space
\def\nthinsp{\mskip -2   mu}
\def\nmedsp {\mskip -2.75mu}
\def\nthiksp{\mskip -3.5 mu}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%  Specially lowered subscripts (see \sub above)
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\Asubk{A\sub{\nthinsp k}}
\def\Bsubk{B\sub{\nthinsp k}}
\def\Fsubk{F\sub{\nmedsp k}}
\def\Gsubk{G\sub{\nthinsp k}}
\def\Hsubk{H\sub{\nthinsp k}}
\def\HsubB{H\sub{\nthinsp  \scriptscriptstyle{B}}}
\def\HsubS{H\sub{\nthinsp  \scriptscriptstyle{S}}}
\def\HsubBS{H\sub{\nthinsp \scriptscriptstyle{BS}}}
\def\Hz{H\sub{\nthinsp \scriptscriptstyle{Z}}}
\def\Jsubk{J\sub{\nmedsp k}}
\def\Psubk{P\sub{\nthiksp k}}
\def\Qsubk{Q\sub{\nthinsp k}}
\def\Vsubk{V\sub{\nmedsp k}}
\def\Vsubone{V\sub{\nmedsp 1}}
\def\Vsubtwo{V\sub{\nmedsp 2}}
\def\Ysubk{Y\sub{\nmedsp k}}
\def\Wsubk{W\sub{\nthiksp k}}
\def\Zsubk{Z\sub{\nthinsp k}}
\def\Zsubi{Z\sub{\nthinsp i}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%  Subscripts
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\submax{_{\max}}
\def\submin{_{\min}}
\def\subminus{_{\scriptscriptstyle -}}
\def\subplus {_{\scriptscriptstyle +}}

\def\A{_{\scriptscriptstyle A}}
\def\B{_{\scriptscriptstyle B}}
\def\C{_{\scriptscriptstyle C}}
\def\D{_{\scriptscriptstyle D}}
\def\E{_{\scriptscriptstyle E}}
\def\F{_{\scriptscriptstyle F}}
\def\G{_{\scriptscriptstyle G}}
\def\H{_{\scriptscriptstyle H}}
\def\I{_{\scriptscriptstyle I}}
\def\J{_{\scriptscriptstyle J}}
\def\K{_{\scriptscriptstyle K}}
\def\L{_{\scriptscriptstyle L}}
\def\M{_{\scriptscriptstyle M}}
\def\N{_{\scriptscriptstyle N}}
\def\O{_{\scriptscriptstyle O}}
\def\P{_{\scriptscriptstyle P}}
\def\Q{_{\scriptscriptstyle Q}}
\def\R{_{\scriptscriptstyle R}}
\def\U{_{\scriptscriptstyle U}}
\def\V{_{\scriptscriptstyle V}}
\def\W{_{\scriptscriptstyle W}}
\def\Y{_{\scriptscriptstyle Y}}
\def\Z{_{\scriptscriptstyle Z}}
\def\w{_w}
\def\k{_k}
\def\kp#1{_{k+#1}}
\def\km#1{_{k-#1}}
\def\j{_j}
\def\jp#1{_{j+#1}}
\def\jm#1{_{j-#1}}
\def\subb{\B}
\def\subc{\C}
\def\subf{\F}
\def\subh{\H}
\def\subk{\K}
\def\subm{\M}
\def\subn{\N}
\def\subp{\P}
\def\subs{_{\scriptscriptstyle S}}
\def\subt{_{\scriptscriptstyle T}}
\def\subr{\R}
\def\subz{\Z}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%  bars, hats, tildes  (\skew4 is the default)
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\alphabar{\bar \alpha}
\def\alphahat{\skew3\hat \alpha}
\def\alphatilde{\skew3\tilde \alpha}
\def\betabar{\skew{2.8}\bar\beta}
\def\betahat{\skew{2.8}\hat\beta}
\def\betatilde{\skew{2.8}\tilde\beta}
\def\deltabar{\bar\delta}
\def\deltilde{\skew5\tilde \delta}
\def\deltatilde{\deltilde}
\def\etabar{\bar\eta}
\def\gammabar{\bar\gamma}
\def\lambar{\bar\lambda}
\def\lamhat{\skew{2.8}\hat \lambda}
\def\lambdahat{\lamhat}
\def\lambdatilde{\tilde{\lambda}}
\def\mubar{\skew3\bar \mu}
\def\muhat{\skew3\hat \mu}
\def\mutilde{\skew3\tilde\mu}
\def\nubar{\skew3\bar\nu}
\def\nuhat{\skew3\hat\nu}
\def\nutilde{\skew3\tilde\nu}
\def\omegabar{\bar\omega}
\def\omegahat{\skew3\hat\omega}
\def\omegatilde{\tilde\omega}
\def\phibar{\bar\phi}
\def\pibar{\bar\pi}
\def\pihat{\skew1\widehat \pi}
\def\sigmaB{\mkern 3mu\overline {\mkern-3mu\sigma\mkern 1mu}\mkern-1mu}
\def\sigmab{\mkern-2mu\underline{\mkern 2mu\sigma\mkern-3mu}\mkern 3mu}
\def\sigmabar{\bar\sigma}
\def\rhobar{\bar\rho}
\def\rhohat{\widehat\rho}
\def\taubar{\bar\tau}
\def\tautilde{\tilde\tau}
\def\tauhat{\hat\tau}
\def\thetabar{\bar\theta}
\def\xibar{\skew4\bar\xi}

\def\abar{\skew3\bar a}
\def\ahat{\skew2\widehat a}
\def\atilde{\skew2\widetilde a}
\def\Abar{\skew7\bar A}
\def\Ahat{\widehat A}
\def\Atilde{\widetilde A}
\def\bbar{\skew3\bar b}
\def\bhat{\skew2\widehat b}
\def\btilde{\skew2\widetilde b}
\def\Bbar{\bar B}
\def\Bhat{\widehat B}
\def\cbar{\skew3\bar c}
\def\chat{\skew3\widehat c}
\def\ctilde{\widetilde c}
\def\Cbar{\bar C}
\def\Chat{\widehat C}
\def\Ctilde{\widetilde C}
\def\dbar{\bar d}
\def\dhat{\widehat d}
\def\dtilde{\widetilde d}
\def\Dbar{\bar D}
\def\Dhat{\widehat D}
\def\Dtilde{\widetilde D}
\def\ehat{\skew3\widehat e}
\def\ebar{\bar e}
\def\Ebar{\bar E}
\def\Ehat{\widehat E}
\def\Etilde{\widetilde E}
\def\fbar{\bar f}
\def\fhat{\widehat f}
\def\ftilde{\widetilde f}
\def\Fbar{\bar F}
\def\Fhat{\widehat F}
\def\Ftilde{\widetilde F}
\def\gbar{\skew{4.3}\bar g}
\def\ghat{\skew{3}\widehat g}
\def\gtilde{\skew{4.5}\widetilde g}
\def\Gbar{\bar G}
\def\Ghat{\widehat G}
%\def\hbar{\skew{4.2}\bar h}
\def\hhat{\skew2\widehat h}
\def\htilde{\skew3\widetilde h}
\def\Hbar{\skew5\bar H}
\def\Hhat{\widehat H}
\def\Htilde{\widetilde H}
\def\Ibar{\skew5\bar I}
\def\Itilde{\widetilde I}
\def\Jbar{\skew6\bar J}
\def\Jhat{\widehat J}
\def\Jtilde{\widetilde J}
\def\kbar{\skew{4.4}\bar k}
\def\Khat{\widehat K}
\def\Kbar{\skew{4.4}\bar K}
\def\Ktilde{\widetilde K}
\def\ellbar{\bar \ell}
\def\lhat{\skew2\widehat l}
\def\lbar{\skew2\bar l}
\def\Lbar{\skew{4.3}\bar L}
\def\Lhat{\widehat L}
\def\Ltilde{\widetilde L}
\def\mbar{\skew2\bar m}
\def\mhat{\widehat m}
\def\Mbar{\skew{4.4}\bar M}
\def\Mhat{\widehat M}
\def\Mtilde{\widetilde M}
\def\Nbar{\skew{4.4}\bar N}
\def\Ntilde{\widetilde N}
\def\nbar{\skew2\bar n}
\def\pbar{\skew2\bar p}
\def\phat{\skew2\widehat p}
\def\ptilde{\skew2\widetilde p}
\def\Pbar{\skew5\bar P}
\def\Phat{\widehat P}
\def\Ptilde{\skew5\widetilde P}
\def\qbar{\bar q}
\def\qhat{\skew2\widehat q}
\def\qtilde{\widetilde q}
\def\Qbar{\bar Q}
\def\Qhat{\widehat Q}
\def\Qtilde{\widetilde Q}
\def\rbar{\skew3\bar r}
\def\rhat{\skew3\widehat r}
\def\rtilde{\skew3\widetilde r}
\def\Rbar{\skew5\bar R}
\def\Rhat{\widehat R}
\def\Rtilde{\widetilde R}
\def\sbar{\bar s}
\def\shat{\widehat s}
\def\stilde{\widetilde s}
\def\Shat{\widehat S}
\def\Sbar{\skew2\bar S}
\def\tbar{\bar t}
\def\ttilde{\widetilde t}
\def\that{\widehat t}
\def\Tbar{\bar T}
\def\That{\widehat T}
\def\Ttilde{\widetilde T}
\def\ubar{\skew3\bar u}
\def\uhat{\skew3\widehat u}
\def\utilde{\skew3\widetilde u}
\def\Ubar{\skew2\bar U}
\def\Uhat{\widehat U}
\def\Utilde{\widetilde U}
\def\vbar{\skew3\bar v}
\def\vhat{\skew3\widehat v}
\def\vtilde{\skew3\widetilde v}
\def\Vbar{\skew2\bar V}
\def\Vhat{\widehat V}
\def\Vtilde{\widetilde V}
\def\wbar{\skew3\bar w}
\def\what{\skew3\widehat w}
\def\wtilde{\skew3\widetilde w}
\def\Wbar{\skew3\bar W}
\def\What{\widehat W}
\def\Wtilde{\widetilde W}
\def\xbar{\bar{x}}
\def\xhat{\skew{2.8}\widehat x}
\def\xtilde{\skew3\widetilde x}
\def\Xhat{\widehat X}
\def\ybar{\skew3\bar y}
\def\yhat{\skew2\widehat y}
\def\ytilde{\skew3\widetilde y}
\def\Ybar{\skew2\bar Y}
\def\Yhat{\widehat Y}
\def\zbar{\skew{2.8}\bar z}
\def\zhat{\skew{2.8}\widehat z}
\def\ztilde{\skew{2.8}\widetilde z}
\def\Zbar{\skew5\bar Z}
\def\Zhat{\widehat Z}
\def\Ztilde{\widetilde Z}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%  Stars
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\lamstar{\lambda^*}
\def\lamstark{\lambda^*\k}
\def\lambarstark{\lambar^*\k}
\def\pistar{\pi^*}
\def\pistark{\pi^*_k}
\def\rhostar{\rho^*}
\def\mustar{\mu^*}
\def\taustar{\tau^*}
\def\cstar{c^*}
\def\dstar{d^*}
\def\gstar{g^*}
\def\Jstar{J^*}
\def\pstar{p^*}
\def\rstar{r^*}
\def\rstark{r^*\k}
\def\vstar{v^*}
\def\vstark{v^*\k}
\def\wstar{w^*}
\def\wstark{w^*\k}
\def\xstar{x^*}
\def\xstarhatk{\hat x^*\k}
\def\xstark{x^*\k}
\def\xstarzero{x^*_0}
\def\xstarkm1{x^*\km1}
\def\ystar{y^*}
\def\ystarhatk{\hat y^*\k}
\def\ystark{y^*\k}
\def\ystarkm1{y^*\km1}
\def\zstar{z^*}
\def\zstark{z^*\k}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%  Math italic fonts
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\mit{\mathit}
\def\Deltait{{\mit \Delta}}
\def\Gammait{{\mit \Gamma}}
\def\Lambdait{{\mit \Lambda}}
\def\Sigmait{{\mit \Sigma}}
\def\Lambarit{\skew5\bar{\mit \Lambda}}
\def\Omegait{{\mit \Omega}}
\def\Omegaitbar{\skew5\bar{\mit \Omega}}
\def\Thetait{{\mit \Theta}}
\def\Piitbar{\skew5\bar{\mit \Pi}}
\def\Piit{{\mit \Pi}}
\def\Phiit{{\mit \Phi}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%  Math calligraphy fonts
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\lscr{\ell}
\def\lscrbar{\ellbar}
\def\Ascr{\mathcal{A}}
\def\Bscr{\mathcal{B}}
\def\Cscr{\mathcal{C}}
\def\Escr{\mathcal{E}}
\def\Fscr{\mathcal{F}}
\def\Dscr{\mathcal{D}}
\def\Iscr{\mathcal{I}}
\def\Jscr{\mathcal{J}}
\def\Kscr{\mathcal{K}}
\def\Lscr{\mathcal{L}}
\def\Mscr{\mathcal{M}}
\def\Nscr{\mathcal{N}}
\def\Oscr{\mathcal{O}}
\def\Pscr{\mathcal{P}}
\def\Qscr{\mathcal{Q}}
\def\Rscr{\mathcal{R}}
\def\Sscr{\mathcal{S}}
\def\Tscr{\mathcal{T}}
\def\Uscr{\mathcal{U}}
\def\Vscr{\mathcal{V}}
\def\Wscr{\mathcal{W}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%  Delta quantities
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\dd{\Deltait d}
\def\dx{\Deltait x}
\def\dy{\Deltait y}
\def\dz{\Deltait z}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Computer packages
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\Matlab{\textsc{Matlab}}
\newcommand{\code}[1]{{\small#1}}
\def\KNOSSOS{\code{KNOSSOS}}
\def\MINOS  {\code{MINOS}}
\def\LANCE  {\code{LANCELOT}}
\def\SNOPT  {\code{SNOPT}}
\def\SLQP   {S$\ell_1$QP}
\def\QPSOL  {\code{QPSOL}}
\def\LUSOL  {\code{LUSOL}}
\def\LSSOL  {\code{LSSOL}}
\def\GAMS   {\code{GAMS}}
\def\AMPL   {\code{AMPL}}
\def\COPS   {\code{COPS}}
\def\CUTE   {\code{CUTE}}
\def\CUTEr  {\code{CUTEr}}
\def\ADIC   {\code{ADIC}}
\def\CONOPT {\code{CONOPT}}
\def\NEOS   {\code{NEOS}}
\def\cpp    {C\raisebox{0.1ex}{\hbox{\small++}}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Abbreviations
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\Sec{\S}
\def\seq#1{\ensuremath{\{#1\}}}
\newcommand{\e}[1]{\ensuremath{\mathrm{e#1}}} % scientific not. (e)
\def\Tr{\mathop{\hbox{Tr}}}

